WorldSense: A Synthetic Benchmark for Grounded Reasoning in Large Language Models

We propose WorldSense, a benchmark designed to assess the extent to which LLMs are consistently able to sustain tacit world models, by testing how they draw simple inferences from descriptions of simple arrangements of entities. Worldsense is a synthetic benchmark with three problem types, each with their own trivial control, which explicitly avoids bias by decorrelating the abstract structure of problems from the vocabulary and expressions, and by decorrelating all problem subparts with the correct response. We run our benchmark on three state-of-the-art chat-LLMs (GPT3.5, GPT4 and Llama2-chat) and show that these models make errors even with as few as three objects. Furthermore, they have quite heavy response biases, preferring certain responses irrespective of the question. Errors persist even with chain-of-thought prompting and in-context learning. Lastly, we show that while finetuning on similar problems does result in substantial improvements -- within- and out-of-distribution -- the finetuned models do not generalise beyond a constraint problem space.

==> 5-experiments.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% EXPERIMENT 1 %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiment 1. Testing chat LLMs}\label{sec:exp1}
Here, we report the results of the experiment run on three chat-LLMs.

\subsection{Method}

We test OpenAI's GPT3.5 (\textttt{gpt-3.5-turbo}),  GPT4 (\textttt{gpt-4}) using the OpenAI API (we use the default parameters of the interface for chat generation; the experiments were run between august and october 2023). 
In addition, we test Llama2-chat, the chat version of Llama2 70B (HugginFace's \textttt{Llama-2-70b-chat-hf}) by running the inference directly (greedy decoding, temperature 0). 
We feed the prompt to the model as if typed by a user, and recover the generated text. Each problem instance is fed as a new conversation. To evaluate the response of the model, we select the last word of the generated text and normalize it by upcasing and removing extra punctuation. 
If this does not match the set of acceptable answers as specified in the prompt (e.g. \textttt{TRUE} or \textttt{FALSE}), the model receives a continued  conversation where the user asks: ``\textit{What is the final answer? Respond only using one of these possible answers: TRUE, FALSE}".  If the final answer correspond to the ground truth, the model is deemed correct, and incorrect otherwise.

To analyse the results, we first compute \textit{accuracies} on a tuple by tuple basis. We set the trial's accuracy as $1$ if the responses matches the ground truth, $0$ otherwise, and average this score within a tuple. For the completeness problems, we fold the three-way forced choice into a binary choice (responses 1 and 2 are folded as \texttt{KNOWN}, and response 3 as \textttt{UNKNOWN}). To obtained a balanced score, we compute a weighted average where the trials corresponding to \textttt{KNOW} are given a weight of 0.5 and the trials corresponding to \textttt{UNKNOWN} a weight of 1. After such averaging and rebalancing, all of the accuracies across tuples and problem types have a chance level of 0.5.  We also introduce a \textit{response bias} score, computed as follows: all responses \textttt{TRUE}, \textttt{POSSIBLE} or \textttt{KNOWN} are given a score of $1$ (positive poalrity), while \texttt{FALSE}, \texttt{IMPOSSIBLE} or \textttt{UNKNOWN} are given a score of $-1$ (negative polarity). The scores are averaged within tuple (using the same weigthts as above), giving rise to a bias score per tuple in which 0 means absence of bias, and 1 or -1 a strong bias to systematically respond one of the response category. 
\input{tables/summary_table}

\subsection{Results}

In Table \ref{tab:exp1_summary}, we report the accuracies of the three models under consideration on our base task and trivial control experiment. Overall, GPT4 is performing better than GPT3.5 and Llama2-chat, which are barely above chance level. The 'epistemic' problems (consistency and completeness) yield systematically lower performances than the grounded inferences across models. The trivial control shows that a large fraction of the error is due to (tacit) world state generation, but there remain problems in question answering, especially for models other than GPT4. 

Detailed results split up by problem difficulty and number of objects in the described world are in the Supplementary Table \ref{tab:sup_monster_acc} and show that all models make more errors with problems with larger number of entities and struggle with ternary relations (as the performance decreases with problem complexity and/or presence of ternary relations in the query). 
In \cref{tab:supp-skins}, we also show the average error rate across the different skins 
enabling a measure of the model's consistency; in particular, we find that among the different domains, the temporal is the most difficult, and the scalar the easiest. 
Finally, Table \ref{tab:sup_monster_acc} shows that models can be heavily biased in their responses, preferring some responses polarities. 
This is especially true of the chatLLama model which prefers to answer \textttt{FALSE}, \textttt{POSSIBLE} and \textttt{KNOWN} irrespective of the ground truth, the bias being stronger for the normal than the trivial version of each problem type (we definea strong bias has an amplitude of more than .6, which corresponds to 80\% of the response being of one particular polarity). 
The GPT models generally display less bias (only GPT4 has a strong \textttt{KNOW} bias).


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% EXPERIMENT 2 %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experiment 2: in-context learning and chain of though}\label{sec:exp2}
\input{tables/exp2_incontextandCOT_table}

In our second experiment, we evaluate well known methods to improve the reasoning abilities of LLMs: in-context learning and chain-of-thought (COT).
In-context learning consists in prompting the model with a small number of sample problems together with their solution, and chain-of-though enables the model to use its own output to break down a complex problem in smaller ones.


\subsection{Method}
Regarding COT, we replace the final instructions sent to the model. For inference problems: \textit{"Reason step by step; write down your general strategy for solving this question; execute your steps; verify your reasoning, and revise strategy if this does not work. After doing all this reasoning, state your final answer with the sentence: 'The final response is:' followed by one of these 2 options: 'TRUE', 'FALSE', without adding anything more."}. We present similarly the desired responses for the two other classes of problems (consistency and completeness). 

Regarding in-context learning, we prepend the test problem with 5 problems together their the correct response. We test two conditions. In the in-distribution condition (IID), where problems are generated with the same parameters as the test problem (same problem size, same complexity, same skin, same domain). In the out-of-domain distribution (OOD), the sample problems have a different skin and domain (although the same number of entities and complexity). 


\subsection{Results}

As shown in Table  \ref{tab:exp2-incontCOT}, GPT models benefit from COT (4.3\% and 4.6\% absolute for GPT3.5 and GPT4 resp.). Llama2 only shows a trend in the same direction (0.6\%, within the confidence interval). None of the models benefit  from in-context learning, with within-confidence interval fluctuations around the base score, except for GPT3.5 and Llama2 which show a small decrement for IID examples (-3.2\% and -1.6\% resp). Further analyses (Table~\ref{tab:supp_bias_exp2}) show that COT 
systematically decreases the bias for the Llama2 model (going from an average amplitude of .6 down to .3) but has little effect on GPT models where bias amplitude remains small (between .1 and .2). In-context learning induce smaller and less systematic changes in bias.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%% EXPERIMENT 2 %%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Experiment 3: fine tuning}\label{sec:exp3}
In this experiment, we test whether chat models can learn grounded inferences by adding examples in the fine tuning set. In particular we test whether models generalize, by specifically manipulating the similarity between the training set and the test set. 


\subsection{Method}
We build a new training set consisting of problems similar to these described in Section \ref{sec:benchmark} with the following changes. First, all entities are novel. Second, the training set selected 8 of the 18 skins in the test set to be 'in-domain' (4 of the scalar and 4 of the temporal skins, none of the spatial skins). They were populated with novel entities and used to generate 'in-domain' training examples. To increase diversity, we also created 10 entirely new skins (5 scalar and 5 temporal) with new entities and backstories. This set of 18 skins (in two domain) was used to build three training sets of increasing sizes: 10k samples, 100k samples, and 1M samples, each larger set containing the smaller ones. 

We fine tuned both Llama2 7b and Llama2 70b models, by merging our training set with the standard Llama2 instruction fine tuning set \cite{llama2} for X epochs.

For analysis, we run the standard \WS{} test set, which we subdivide into two subsets, in-domain and out-of-domain depending on whether the skins were shared with the training set. 
The oo-domain subset contained therefore 2 scalar and 2 temporal skins plus the entire spatial domain (6 skins), which were never seen during training. 
The difference in performance between these two subsets is intended to measure the extent to which the models learned domain-specific reasoning schemata, or generalize across the abstract class of problems. 
In addition, we introduce four test sets varying in proximity with the training set. 
(1) the memorization test set (memorization) contains the entirety of the 10k samples. 
This is intended to test the extent to which the model memorizes the exact examples given during fine tuning. 
(2) the length generalization test set (out-of-length) contains problems of size 6, intended to test whether what has been learned during fine tuning extends to problems with more objects (3) the question generalization test set (out-of-question), contains queries with a completely new set of queries. 
Instead of asking about the truth value of binary or ternary relations, this set asks questions with unary operators (min or max). 
For instance "the pyramid is the leftmost object". 
This is intended to test whether the models learn to reason about linear order, or just respond to our specific sets of questions (4) the problem generalization test set (out-of-problem) contains a completely different set of problem which does not correspond to an underlying total order. 
In this new set of problems, we use a geometric setting with two binary operators: parallel and perpendicular, which can only be solved in a two-dimensional representation. 
This is intended to test whether fine tuning on linear order problems can boost reasoning beyond linear order. 
Finally, we also test our fine tuned models on standard reasoning tasks (MMLU, GSM8K and MATH). 

\input{tables/exp3_finetuning_table}

\subsection{Results}

As shown in Table \ref{tab:exp3-finetuning}, the fine tuned models improve their performance on \WS{}, both in-domain and out-of-domain, without strong evidence for memorization. The performance shows generalization across problem length, but does not seem to generalize across problem types or to external benchmarks.


==> tables/exp2_incontextandCOT_table.tex <==

\begin{table*}[]
\caption{{\bf Effect of in-context learning and chain of thoughts.} Accuracies achieved by Chain of Thought (COT) and in-context learning (IC: 5 examples most similar to the final query. IID: same nb of entities, complexity, exact same skin. DC: different domain). Results are bolded when better than the normal prompting condition of Experiment 1. Results are given for three LLMs across the three \WS{} problem types and their trivial controls (averaged across lengths 3,4,5). Accuracies are given with 95\% confidence intervals, and chance level is 50\%.}\label{tab:exp2-incontCOT}
\setlength{\tabcolsep}{2.1pt}

%\begin{tabular}{l lll c lll c lll}
%\toprule
% &\multicolumn{3}{c}{GPT-3.5} && \multicolumn{3}{c}{GPT-4} && \multicolumn{3}{c}{ChatLLama-2} \\
% \cline{2-4} \cline{6-8} \cline{10-12}
% Problem&   direct & incont-5 & COT && direct &incont-5 & COT && direct &incont-5 & COT \\
%\hline
%{Inference {\tiny (trivial)}} & 29.8 {\tiny $\pm 3.2$} &xx.x {\tiny $\pm x.x$}& 22.2 {\tiny $\pm 4.1$} && 5.6 {\tiny $\pm 1.9$}  &xx.x {\tiny $\pm x.x$}&  3.1 {\tiny $\pm 2.0$} && 33.3 {\tiny $\pm 4.9$} &xx.x {\tiny $\pm x.x$}& 29.4 {\tiny $\pm 6.7$} \\
%{Inference {\tiny (normal)}}  & 41.6 {\tiny $\pm 2.0$} &xx.x {\tiny $\pm x.x$}& 37.8 {\tiny $\pm 2.8$} && 17.9 {\tiny $\pm 1.8$} &xx.x {\tiny $\pm x.x$}&  8.6 {\tiny $\pm 1.9$} && 35.2 {\tiny $\pm 2.8$} &xx& 35.7 {\tiny $\pm 4.0$} \\
%{Consist. {\tiny (trivial)}}  & 46.8 {\tiny $\pm 2.0$} &xx.x {\tiny $\pm x.x$}& 45.3 {\tiny $\pm 2.8$} && 23.4 {\tiny $\pm 2.0$} &xx.x {\tiny $\pm x.x$}& 14.7 {\tiny $\pm 2.4$} && 44.6 {\tiny $\pm 3.0$} &xx& 48.0 {\tiny $\pm 4.2$} \\
%{Consist. {\tiny (normal)}}   & 50.2 {\tiny $\pm 2.0$} &xx.x {\tiny $\pm x.x$}& 48.4 {\tiny $\pm 2.8$} && 27.4 {\tiny $\pm 2.1$} &xx.x {\tiny $\pm x.x$}& 17.1 {\tiny $\pm 2.5$} && 49.1 {\tiny $\pm 3.0$} &xx& 52.2 {\tiny $\pm 4.2$} \\
%{Complet. {\tiny (trivial)}}  & 40.6 {\tiny $\pm 2.8$} &xx.x {\tiny $\pm x.x$}& 34.8 {\tiny $\pm 3.8$} && 3.4 {\tiny $\pm 1.2$}  &xx.x {\tiny $\pm x.x$}&  4.6 {\tiny $\pm 4.0$} && 30.4 {\tiny $\pm 3.9$} &xx& 29.3 {\tiny $\pm 5.4$} \\
%{Complet. {\tiny (normal)}}   & 46.0 {\tiny $\pm 2.8$} &xx.x {\tiny $\pm x.x$}& 44.1 {\tiny $\pm 4.0$} && 25.5 {\tiny $\pm 2.9$} &xx.x {\tiny $\pm x.x$}& 16.7 {\tiny $\pm 7.1$} && 34.3 {\tiny $\pm 4.0$} &xx& 40.0 {\tiny $\pm 5.9$} \\
% \hline
%Average  & 42.5 {\tiny $\pm x.x$} &xx.x {\tiny $\pm x.x$}& 38.8 {\tiny $\pm x.x$} && 17.2 {\tiny $\pm x.x$} &xx.x {\tiny $\pm x.x$}& 10.8 {\tiny $\pm x.x$} && 37.8 {\tiny $\pm x.x$} &xx& 39.1 {\tiny $\pm x.x$} \\
% \bottomrule
%\end{tabular}

%\begin{tabular}{lllllllllllll}
%\toprule
% & \multicolumn{4}{c}{GPT-3.5} & \multicolumn{4}{c}{GPT-4} & \multicolumn{4}{c}{chatllama2-70b} \\
%Problem & direct & COT & IC-IID & IC-DC & direct & COT & IC-IID & IC-DC & direct & COT & IC-IID & IC-DC \\
%\hline
%Infer. {\tiny (trivial)} & 64.5 {\tiny $\pm 1.1$} & 71.4 {\tiny $\pm 3.5$} & 56.1 {\tiny $\pm 3.4$} & 65.4 {\tiny $\pm 3.5$} & 90.2 {\tiny $\pm 0.7$} & 89.6 {\tiny $\pm 2.2$} & 92.4 {\tiny $\pm 1.9$} & 92.0 {\tiny $\pm 2.0$} & 61.9 {\tiny $\pm 0.8$} & 69.3 {\tiny $\pm 3.1$} & 58.3 {\tiny $\pm 2.6$} & 63.9 {\tiny $\pm 2.4$} \\
%Infer. {\tiny (normal)} & 54.9 {\tiny $\pm 0.6$} & 58.9 {\tiny $\pm 2.0$} & 54.1 {\tiny $\pm 1.9$} & 54.5 {\tiny $\pm 2.0$} & 74.9 {\tiny $\pm 0.6$} & 81.7 {\tiny $\pm 1.7$} & 73.0 {\tiny $\pm 1.8$} & 71.0 {\tiny $\pm 1.8$} & 58.7 {\tiny $\pm 0.4$} & 58.6 {\tiny $\pm 1.9$} & 58.5 {\tiny $\pm 1.4$} & 57.6 {\tiny $\pm 1.4$} \\
%Consist. {\tiny (trivial)} & 52.1 {\tiny $\pm 0.6$} & 55.3 {\tiny $\pm 1.8$} & 49.3 {\tiny $\pm 1.9$} & 51.3 {\tiny $\pm 1.9$} & 70.9 {\tiny $\pm 0.6$} & 76.1 {\tiny $\pm 1.8$} & 70.4 {\tiny $\pm 1.7$} & 71.7 {\tiny $\pm 1.7$} & 53.9 {\tiny $\pm 0.4$} & 51.3 {\tiny $\pm 1.7$} & 50.5 {\tiny $\pm 1.2$} & 51.8 {\tiny $\pm 1.1$} \\
%Consist. {\tiny (normal)} & 50.0 {\tiny $\pm 0.7$} & 50.8 {\tiny $\pm 2.1$} & 48.0 {\tiny $\pm 1.9$} & 51.0 {\tiny $\pm 2.0$} & 64.8 {\tiny $\pm 0.6$} & 69.6 {\tiny $\pm 1.9$} & 61.5 {\tiny $\pm 1.7$} & 64.9 {\tiny $\pm 1.7$} & 49.4 {\tiny $\pm 0.3$} & 49.3 {\tiny $\pm 1.6$} & 49.9 {\tiny $\pm 1.1$} & 49.3 {\tiny $\pm 0.9$} \\
%Complet. {\tiny (trivial)} & 59.7 {\tiny $\pm 0.9$} & 68.8 {\tiny $\pm 2.8$} & 56.1 {\tiny $\pm 2.5$} & 53.3 {\tiny $\pm 2.4$} & 92.5 {\tiny $\pm 0.6$} & 94.5 {\tiny $\pm 1.6$} & 95.0 {\tiny $\pm 1.4$} & 94.0 {\tiny $\pm 1.5$} & 60.1 {\tiny $\pm 0.7$} & 60.1 {\tiny $\pm 2.9$} & 57.0 {\tiny $\pm 1.9$} & 54.1 {\tiny $\pm 1.4$} \\
%Complet. {\tiny (normal)} & 51.7 {\tiny $\pm 1.0$} & 53.4 {\tiny $\pm 3.2$} & 50.1 {\tiny $\pm 2.2$} & 51.3 {\tiny $\pm 2.2$} & 58.1 {\tiny $\pm 0.6$} & 67.5 {\tiny $\pm 2.7$} & 61.8 {\tiny $\pm 2.5$} & 63.7 {\tiny $\pm 2.5$} & 51.4 {\tiny $\pm 0.5$} & 50.4 {\tiny $\pm 2.5$} & 51.5 {\tiny $\pm 1.2$} & 50.7 {\tiny $\pm 1.0$} \\
%\hline
%Avg & 55.5 {\tiny $\pm 0.4$} & 59.8 {\tiny $\pm 1.4$} & 52.3 {\tiny $\pm 1.3$} & 54.5 {\tiny $\pm 1.3$} & 75.2 {\tiny $\pm 0.4$} & 79.8 {\tiny $\pm 1.2$} & 75.7 {\tiny $\pm 1.2$} & 76.2 {\tiny $\pm 1.2$} & 55.9 {\tiny $\pm 0.3$} & 56.5 {\tiny $\pm 1.2$} & 54.3 %{\tiny $\pm 0.9$} & 54.6 {\tiny $\pm 0.8$} \\
%\bottomrule
%\end{tabular}

\begin{tabular}{l lll c lll c lll}
\toprule
 & \multicolumn{3}{c}{GPT-3.5} && \multicolumn{3}{c}{GPT-4} && \multicolumn{3}{c}{chatllama2-70b} \\
 \cline{2-4} \cline{6-8} \cline{10-12}
Problem & COT & IC-IID & IC-DC && COT & IC-IID & IC-DC && COT & IC-IID & IC-DC \\
\hline

Infer. {\tiny (trivial)}  &\bf 71.4 {\tiny $\pm 3.5$} & 56.1 {\tiny $\pm 3.4$} &\bf 65.4 {\tiny $\pm 3.5$} &&    89.6 {\tiny $\pm 2.2$} &\bf 92.4 {\tiny $\pm 1.9$} &\bf 92.0 {\tiny $\pm 2.0$} &&\bf 69.3 {\tiny $\pm 3.1$} & 58.3 {\tiny $\pm 2.6$} &\bf 63.9 {\tiny $\pm 2.4$} \\
Infer. {\tiny (normal)}   &\bf 58.9 {\tiny $\pm 2.0$} & 54.1 {\tiny $\pm 1.9$} &    54.5 {\tiny $\pm 2.0$} &&\bf 81.7 {\tiny $\pm 1.7$} &    73.0 {\tiny $\pm 1.8$} &   71.0 {\tiny $\pm 1.8$} && 58.6 {\tiny $\pm 1.9$} & 58.5 {\tiny $\pm 1.4$} & 57.6 {\tiny $\pm 1.4$} \\
Consist. {\tiny (trivial)}&\bf 55.3 {\tiny $\pm 1.8$} & 49.3 {\tiny $\pm 1.9$} &    51.3 {\tiny $\pm 1.9$} &&\bf 76.1 {\tiny $\pm 1.8$} &    70.4 {\tiny $\pm 1.7$} &\bf 71.7 {\tiny $\pm 1.7$} && 51.3 {\tiny $\pm 1.7$} & 50.5 {\tiny $\pm 1.2$} & 51.8 {\tiny $\pm 1.1$} \\
Consist. {\tiny (normal)} &\bf 50.8 {\tiny $\pm 2.1$} & 48.0 {\tiny $\pm 1.9$} &\bf 51.0 {\tiny $\pm 2.0$} &&\bf 69.6 {\tiny $\pm 1.9$} &    61.5 {\tiny $\pm 1.7$} &\bf 64.9 {\tiny $\pm 1.7$} && 49.3 {\tiny $\pm 1.6$} &\bf 49.9 {\tiny $\pm 1.1$} & 49.3 {\tiny $\pm 0.9$} \\
Complet. {\tiny (trivial)}&\bf 68.8 {\tiny $\pm 2.8$} & 56.1 {\tiny $\pm 2.5$} &    53.3 {\tiny $\pm 2.4$} &&\bf 94.5 {\tiny $\pm 1.6$} &\bf 95.0 {\tiny $\pm 1.4$} &\bf 94.0 {\tiny $\pm 1.5$} && 60.1 {\tiny $\pm 2.9$} & 57.0 {\tiny $\pm 1.9$} & 54.1 {\tiny $\pm 1.4$} \\
Complet. {\tiny (normal)} &\bf 53.4 {\tiny $\pm 3.2$} & 50.1 {\tiny $\pm 2.2$} &    51.3 {\tiny $\pm 2.2$} &&\bf 67.5 {\tiny $\pm 2.7$} &\bf 61.8 {\tiny $\pm 2.5$} &\bf 63.7 {\tiny $\pm 2.5$} && 50.4 {\tiny $\pm 2.5$} &\bf 51.5 {\tiny $\pm 1.2$} & 50.7 {\tiny $\pm 1.0$} \\

\hline
Avg. trivial &\bf 65.4 {\tiny $\pm 2.0$} & 53.9 {\tiny $\pm 1.8$} & 56.9 {\tiny $\pm 1.9$} &&\bf  87.1 {\tiny $\pm 1.5$} &\bf 86.2 {\tiny $\pm 1.5$} &\bf 86.2 {\tiny $\pm 1.5$} &&\bf 60.0 {\tiny $\pm 1.9$} & 55.4 {\tiny $\pm 1.3$} & 56.8 {\tiny $\pm 1.2$} \\
Avg. normal &\bf 54.5 {\tiny $\pm 2.0$} & 51.1 {\tiny $\pm 1.8$} & 52.4 {\tiny $\pm 1.8$} &&\bf  73.1 {\tiny $\pm 1.8$} & 65.8 {\tiny $\pm 1.8$} & 66.7 {\tiny $\pm 1.7$} && 52.6 {\tiny $\pm 1.7$} & 53.4 {\tiny $\pm 1.2$} & 52.6 {\tiny $\pm 1.1$} \\

\it Grand Average                       &\bf \textit{59.8} {\tiny $\pm 1.4$} &\it 52.3 {\tiny $\pm 1.3$} &\it    54.5 {\tiny $\pm 1.3$} &&\bf \textit{79.8} {\tiny $\pm 1.2$} &\bf \textit{75.7} {\tiny $\pm 1.2$} &\bf \textit{76.2} {\tiny $\pm 1.2$} &&\bf \textit{56.5} {\tiny $\pm 1.2$} &\it 54.3 {\tiny $\pm 0.9$} &\it 54.6 {\tiny $\pm 0.8$} \\
\bottomrule
\end{tabular}


\end{table*}





==> tables/exp3_finetuning_table.tex <==
\begin{table*}[]
\caption{{\bf Fine tuning results}. Llama2-7B and a Llama2-70B models are fine tuned with an instruction following dataset plus varying amounts of samples from the WorldSense training set (10k, 100k, 1M samples, each larger set containing the smaller ones). Accuracies are averaged across the 3 types of problems in both the trivial and normal version. The memorization test set contains the same samples as the 10k training set. The test set is splitted into in-domain (ind) and out-of-domain (ood), based on whether the operators are in the training set or not. The generalization test set contains test set problems with length 6 (oo-length), same domain problems but with novel questions (oo-quest.), or completely new problems not involving linear order (oo-prob.). Also shown is results on a standard reasoning dataset (MLLU). Accuracies are given with 95\% confidence intervals.}\label{tab:exp3-finetuning}
\setlength{\tabcolsep}{2pt}
\centering
\begin{tabular}{l c ccc c ccc c}

\toprule
&              & \multicolumn{3}{c}{\WS}        && \multicolumn{3}{c}{Generalization}       &        \\
\cline{3-5}\cline{7-9}
Model& Memor. & {Avg} & {(ind.)} & {(ood)} && oo-length & {oo-quest.} & {oo-prob.} & {MMLU} \\

%Model    & Memor. & WS Benchmark & {\tiny $\pm (ind)$} & {\tiny $\pm (ood)$} & oo-length & oo-quest & oo-prob & MMLU\\
\hline
Llama2$_{7B}$-FT & 50.7 {\tiny $\pm 0.5$} & 50.7 {\tiny $\pm 0.5$} & 51.2 {\tiny $\pm 0.7$} & 50.3 {\tiny $\pm 0.6$} && 50.2 {\tiny $\pm 0.5$} \\
Llama2$_{7B}$-FT+2k & 50.6 {\tiny $\pm 0.5$} & 50.6 {\tiny $\pm 0.4$} & 50.5 {\tiny $\pm 0.7$} & 50.6 {\tiny $\pm 0.5$} && 50.7 {\tiny $\pm 0.5$} \\
Llama2$_{7B}$-FT+10k & 54.2 {\tiny $\pm 0.7$} & 52.8 {\tiny $\pm 0.5$} & 52.8 {\tiny $\pm 0.8$} & 53.0 {\tiny $\pm 0.7$} && 53.7 {\tiny $\pm 0.7$} \\
Llama2$_{7B}$-FT+100k & 62.1 {\tiny $\pm 0.9$} & 59.6 {\tiny $\pm 0.7$} & 60.8 {\tiny $\pm 1.1$} & 59.1 {\tiny $\pm 0.9$} && 58.6 {\tiny $\pm 0.8$} \\
LLama2$_{7B}$-FT+1M & 68.6 {\tiny $\pm 0.9$} & 65.0 {\tiny $\pm 0.8$} & 68.0 {\tiny $\pm 1.2$} & 63.5 {\tiny $\pm 1.1$} && 63.6 {\tiny $\pm 0.9$} \\
\hline
Llama2$_{70B}$-FT+0 & 56.0 {\tiny $\pm 0.7$} & 54.9 {\tiny $\pm 0.2$} & 56.5 {\tiny $\pm 0.4$} & 53.7 {\tiny $\pm 0.3$} && 53.7 {\tiny $\pm 0.7$} & 53.6 {\tiny $\pm 1.0$} & 61.0 {\tiny $\pm 1.0$} \\
Llama2$_{70B}$-FT+100k & 78.1 {\tiny $\pm 1.0$} & 75.3 {\tiny $\pm 0.4$} & 77.3 {\tiny $\pm 0.5$} & 73.7 {\tiny $\pm 0.5$} && 69.5 {\tiny $\pm 1.0$} & 54.5 {\tiny $\pm 0.8$} & 63.5 {\tiny $\pm 0.7$} \\
Llama2$_{70B}$-FT+1M & 78.4 {\tiny $\pm 1.0$} & 77.4 {\tiny $\pm 0.4$} & 78.6 {\tiny $\pm 0.5$} & 76.4 {\tiny $\pm 0.5$} && 73.7 {\tiny $\pm 1.1$} & 55.3 {\tiny $\pm 1.3$} & 70.3 {\tiny $\pm 0.9$} \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/exp_by_domain.tex <==
\begin{table*}[!h]
\setlength{\tabcolsep}{3.1pt}
\begin{tabular}{llllllllll}
Model & \multicolumn{3}{c}{\bfseries GPT3.5} & \multicolumn{3}{c}{\bfseries GPT4} & \multicolumn{3}{c}{\bfseries ChatLLaMA-2} \\
Domain & \textit{scalar} & \textit{spatial} & \textit{temporal} & \textit{scalar} & \textit{spatial} & \textit{temporal} & \textit{scalar} & \textit{spatial} & \textit{temporal} \\
Problem &  &  &  &  &  &  &  &  &  \\
\textit{Infer}. {\tiny (trivial)} & 68.1 {\tiny $\pm 2.0$} & 61.0 {\tiny $\pm 1.9$} & 65.4 {\tiny $\pm 1.9$} & 97.3 {\tiny $\pm 0.7$} & 88.3 {\tiny $\pm 1.3$} & 85.4 {\tiny $\pm 1.3$} & 72.8 {\tiny $\pm 1.6$} & 60.3 {\tiny $\pm 1.4$} & 53.6 {\tiny $\pm 0.8$} \\
\textit{Infer}. {\tiny (normal)} & 57.7 {\tiny $\pm 1.2$} & 53.7 {\tiny $\pm 1.1$} & 53.8 {\tiny $\pm 1.1$} & 78.4 {\tiny $\pm 1.0$} & 78.4 {\tiny $\pm 1.0$} & 70.1 {\tiny $\pm 1.1$} & 65.6 {\tiny $\pm 1.0$} & 57.1 {\tiny $\pm 0.7$} & 54.7 {\tiny $\pm 0.6$} \\
\textit{Consis}. {\tiny (trivial)} & 54.7 {\tiny $\pm 1.2$} & 51.4 {\tiny $\pm 1.1$} & 50.4 {\tiny $\pm 1.2$} & 77.0 {\tiny $\pm 0.9$} & 72.0 {\tiny $\pm 0.9$} & 64.8 {\tiny $\pm 1.0$} & 56.1 {\tiny $\pm 0.6$} & 56.7 {\tiny $\pm 0.9$} & 49.8 {\tiny $\pm 0.7$} \\
\textit{Consis}. {\tiny (normal)} & 51.0 {\tiny $\pm 1.2$} & 48.9 {\tiny $\pm 1.2$} & 49.9 {\tiny $\pm 1.2$} & 70.2 {\tiny $\pm 1.0$} & 63.9 {\tiny $\pm 1.0$} & 61.0 {\tiny $\pm 1.1$} & 50.3 {\tiny $\pm 0.2$} & 49.0 {\tiny $\pm 0.6$} & 48.8 {\tiny $\pm 0.6$} \\
\textit{Compl}. {\tiny (trivial)} & 59.3 {\tiny $\pm 1.6$} & 60.1 {\tiny $\pm 1.7$} & 60.4 {\tiny $\pm 1.7$} & 97.4 {\tiny $\pm 0.5$} & 92.6 {\tiny $\pm 1.0$} & 89.4 {\tiny $\pm 1.2$} & 62.8 {\tiny $\pm 1.3$} & 57.9 {\tiny $\pm 1.2$} & 60.7 {\tiny $\pm 1.2$} \\
\textit{Compl}. {\tiny (normal)} & 51.3 {\tiny $\pm 1.7$} & 52.4 {\tiny $\pm 1.8$} & 51.7 {\tiny $\pm 1.7$} & 69.4 {\tiny $\pm 1.5$} & 51.7 {\tiny $\pm 0.6$} & 54.3 {\tiny $\pm 0.9$} & 52.6 {\tiny $\pm 0.9$} & 51.6 {\tiny $\pm 0.8$} & 50.3 {\tiny $\pm 0.8$} \\
\end{tabular}
\caption{Accuracy breakdown by domain.}\label{tab:exp1_by_domain}
\end{table*}


==> tables/summary_table.tex <==
\begin{table}[]
\caption{{\bf Accuracies of 3 chat-LLMs on the \WS{} Benchmark (Exp. 1)} for the problem types: grounded inference (Infer.), consistency (Consist.), and completenedd (Complet.). Each problem also has a trivial control version. Accuracies are given with 95\% confidence intervals, chance level at 50\%.}\label{tab:exp1_summary}
\setlength{\tabcolsep}{3pt}

\begin{tabular}{lccc}
\toprule
Problem & \multicolumn{1}{c}{GPT-3.5} & \multicolumn{1}{c}{GPT-4} & \multicolumn{1}{c}{ChLLama-2} \\
\hline
%Infer. {\tiny (trivial)}  & 66.5 {\tiny $\pm 1.9$} & 91.7 {\tiny $\pm 1.4$} & 62.3 {\tiny $\pm 1.9$}   \\
%Infer. {\tiny (normal)}   & 54.1 {\tiny $\pm 1.1$} & 76.1 {\tiny $\pm 1.3$} & 58.9 {\tiny $\pm 1.1$}   \\
%\hline
%Consist. {\tiny (trivial)}& 52.3 {\tiny $\pm 1.1$} & 71.5 {\tiny $\pm 1.3$} & 53.7 {\tiny $\pm 1.1$}  \\
%Consist. {\tiny (normal)} & 49.7 {\tiny $\pm 1.1$} & 64.9 {\tiny $\pm 1.4$} & 50.0 {\tiny $\pm 0.7$}  \\
%\hline
%Complet. {\tiny (trivial)}& 58.5 {\tiny $\pm 1.6$} & 93.0 {\tiny $\pm 1.3$} & 60.5 {\tiny $\pm 1.7$} \\
%Complet. {\tiny (normal)}& 51.0 {\tiny $\pm 1.7$} & 58.1 {\tiny $\pm 1.5$} & 51.7 {\tiny $\pm 1.1$}  \\
%\hline
%Average                   & 55.3 {\tiny $\pm x.x$} & 75.9 {\tiny $\pm x.x$} & 56.2 {\tiny $\pm x.x$}  \\
\multicolumn{4}{c}{\underline{Accuracy}}\\

Infer. {\tiny (trivial)} & 64.5 {\tiny $\pm 1.1$} & 90.2 {\tiny $\pm 0.7$} & 61.9 {\tiny $\pm 0.8$} \\
Infer. {\tiny (normal)} & 54.9 {\tiny $\pm 0.6$} & 74.9 {\tiny $\pm 0.6$} & 58.7 {\tiny $\pm 0.4$} \\
%\hline
Consist. {\tiny (trivial)} & 52.1 {\tiny $\pm 0.6$} & 70.9 {\tiny $\pm 0.6$} & 53.9 {\tiny $\pm 0.4$} \\
Consist. {\tiny (normal)} & 50.0 {\tiny $\pm 0.7$} & 64.8 {\tiny $\pm 0.6$} & 49.4 {\tiny $\pm 0.3$} \\
%\hline
Complet. {\tiny (trivial)} & 59.7 {\tiny $\pm 0.9$} & 92.5 {\tiny $\pm 0.6$} & 60.1 {\tiny $\pm 0.7$} \\
Complet. {\tiny (normal)} & 51.7 {\tiny $\pm 1.0$} & 58.1 {\tiny $\pm 0.6$} & 51.4 {\tiny $\pm 0.5$} \\
\hline
Avg. {\tiny (trivial)} & 59.0 {\tiny $\pm 0.6$} & 84.9 {\tiny $\pm 0.5$} & 59.0 {\tiny $\pm 0.4$} \\
Avg. {\tiny (normal)} & 52.3 {\tiny $\pm 0.6$} & 66.4 {\tiny $\pm 0.6$} & 53.3 {\tiny $\pm 0.4$} \\
\it Grand Avg. &\it 55.5 {\tiny $\pm 0.4$} &\it 75.2 {\tiny $\pm 0.4$} &\it 55.9 {\tiny $\pm 0.3$} \\
\hline
\hline
\multicolumn{4}{c}{\underline{Response Bias}}\\
Infer. {\tiny (trivial)}  & +0.08 & -0.14 & -0.43 \\
Infer. {\tiny (normal)}   & -0.34 & -0.20 & -0.63 \\
Consist. {\tiny (trivial)}& -0.15 & -0.12 & +0.52 \\
Consist. {\tiny (normal)} & \,\,0.00 &  \,\,0.00 & +0.79 \\
Complet. {\tiny (trivial)}& -0.02 & +0.09 & +0.52 \\
Complet. {\tiny (normal)} & +0.20 & +0.78 & +0.83 \\
\hline
Bias Amp. {\tiny (trivial)} & 0.08 & 0.11 & 0.49 \\
Bias Amp. {\tiny (normal)} & 0.18 & 0.33 & 0.75 \\
\it Average Bias Amp.&\it 0.13  &\it 0.22 &\it 0.62 \\
\bottomrule
\end{tabular}

\end{table}


==> ws_test_examples.tex <==
\begin{table*}
\renewcommand{\arraystretch}{1.5}
\small
\begin{tabular}{|p{0.12\textwidth}<{\centering}|p{0.47\textwidth}|p{0.3\textwidth}<{\centering}|}
\hline
\textit{Experiment} & \multicolumn{1}{c|}{\textit{Description}} & \textit{Question} \\
\hline
Grounded Inference (normal)  &   There are 3 objects arranged in a line: the bag is to the right of the box and the table is to the left of the box.
    & \multirow{2}{0.3\textwidth}[-2ex]{Is the following sentence `the table is to the left of the bag' TRUE or FALSE ? Only respond TRUE or FALSE without any explanation. }\\
(trivial control) & There are 3 objects arranged in a line. We list them from left to right: the table, the box, the bag. 
    &  \\
    \hline
    Consistency (normal)  & There are 3 objects arranged in a line. Someone says `the table is to the left of the bag, the table is to the left of the box and the bag is to the right of the box.'  & \multirow{2}{0.3\textwidth}[-2ex]{Is the situation just described possible or impossible ? Only respond with `POSSIBLE' or `IMPOSSIBLE' without any explanation.} \\
    (trivial control) & There are 3 objects arranged in a line.
Someone says: `the book is to the left of the chair, the book is to the right of the mug and the mug is to the left of the chair.'&  \\ \hline
    Completeness (normal)  & There are 3 objects arranged in a line: the ball is to the left of the mug and the chair is to the right of the ball.  &\multirow{2}{0.3\textwidth}[-0ex]{(1) the chair is to the right of the mug; (2) the chair is to the left of the mug; (3) it is impossible to decide. Only respond with one of these options: (1), (2), or (3).}\\
(trivial control)&There are 3 objects arranged in a line: the ball is in front of the mug and the chair is in front of the ball.  & \\
\hline
\end{tabular}
\caption{\textbf{Representative samples for the three problem types of \WS{} with three objects.}}\label{tab:experiment_examples}
\end{table*}

